TIGeR: Tool-Integrated Geometric Reasoning in Vision-Language Models for Robotics

Vision-Language Models (VLMs) have shown remarkable capabilities in spatial reasoning, yet they remain fundamentally limited to qualitative precision and lack the computational precision required for real-world robotics. Current approaches fail to leverage metric cues from depth sensors and camera calibration, instead reducing geometric problems to pattern recognition tasks that cannot deliver the centimeter-level accuracy essential for robotic manipulation. We present TIGeR (Tool-Integrated Geometric Reasoning), a novel framework that transforms VLMs from perceptual estimators to geometric computers by enabling them to generate and execute precise geometric computations through external tools. Rather than attempting to internalize complex geometric operations within neural networks, TIGeR empowers models to recognize geometric reasoning requirements, synthesize appropriate computational code, and invoke specialized libraries for exact calculations. To support this paradigm, we introduce TIGeR-300K, a comprehensive tool-invocation-oriented dataset covering point transformations, pose estimation, and spatial compatibility verification, complete with tool invocation sequences and intermediate computations. Through a two-stage training pipeline combining supervised fine-tuning (SFT) and reinforcement fine-tuning (RFT) with our proposed hierarchical reward design, TIGeR achieves SOTA performance on geometric reasoning benchmarks while demonstrating centimeter-level precision in real-world robotic manipulation tasks.

==> sec/1_introduction.tex <==
\section{Introduction}
% Recent advancements in Vision-Language Models (VLMs) have revolutionized robotic perception and decision-making, enabling robots to interpret visual scenes and execute tasks based on natural language instructions. While current VLMs demonstrate impressive capabilities in spatial reasoning—understanding relative positions, object relationships, and scene layouts—they fundamentally lack the ability to perform geometric reasoning: the precise numerical requirements for real-world robotic applications.
Recent advances in Vision-Language Models (VLMs) have significantly enhanced robotic perception and decision-making, enabling robots to interpret visual scenes and follow natural language instructions. While embodied VLMs exhibit strong spatial reasoning abilities—such as understanding relative positions, object relationships, and scene layouts—they lack the capacity for geometric reasoning, i.e., the precise numerical computations required for real-world manipulation and planning.

Spatial reasoning, as implemented in most embodied VLMs~\cite{fan2025vlm, wu2025spatial, zheng2025learning}, excels at qualitative assessments: determining that an object is ``to the left of'' another, estimating that something is ``about 2 meters away'' or identifying reachable regions. However, geometric reasoning demands quantitative precision: computing exact 3D coordinates for grasping points, calculating rotation matrices for object manipulation, determining spatial compatibility through volume calculations, and generating collision-free trajectories with specific waypoints. These tasks require not just understanding spatial relationships but performing mathematical operations on metric data—a capability fundamentally absent in current VLMs.

This geometric reasoning gap manifests in both perception and output modalities. On the perception side, while depth sensors and stereo cameras can provide precise metric information, existing VLMs~\cite{cheng2024spatialrgpt, liu2025ssr, zhou2025roborefer, cai2025spatialbot} fail to leverage this data effectively. They typically normalize depth values to image-like representations, destroying the metric properties essential for geometric computation. Without access to camera intrinsics and extrinsics, these models cannot transform pixel observations into real-world coordinates, rendering them incapable of the numerical calculations required for precise manipulation.

On the output side, the limitation is even more pronounced. While a handful of VLMs attempt to output 3D positions or bounding boxes~\cite{team2025gemini}, these predictions are statistical approximations learned from data rather than geometric computations grounded in physical measurements. The vast majority of VLMs remain confined to producing 2D pixel coordinates or qualitative descriptions, unable to generate the precise poses, angles, and trajectories that robots need for dexterous manipulation, accurate placement, or optimal path planning.

The core challenge is that geometric reasoning is fundamentally computational, not perceptual. Tasks like calculating grasp poses from point clouds, determining object orientations from multiple views, or planning trajectories that satisfy kinematic constraints require executing mathematical operations on metric data—operations that cannot be learned through pattern recognition alone but must be computed explicitly.

To bridge this gap, we propose \tiger{}: Tool-Integrated Geometric Reasoning, a novel framework that transforms VLMs from spatial estimators into geometric computers. Rather than attempting to internalize geometric computations within neural networks, \tiger{} empowers VLMs to recognize when geometric reasoning is required, formulate the necessary computations as code, and execute these calculations through tool integration. By self-invoking external tools to retrieve camera parameters, depth data, and other metric information, and by generating and executing code for complex geometric operations, \tiger{} enables VLMs to perform the precise numerical reasoning essential for real-world robotic applications.

We curate a comprehensive dataset, \tigerd{}, consisting of 300K samples that span the full spectrum of geometric reasoning tasks—from point transformations and pose calculations to trajectory planning and spatial compatibility checks. Each sample includes not just the task and solution, but the complete tool invocation sequence and computational steps required. Starting from a base VLM, we apply Supervised Fine-Tuning (SFT) to teach the model when and how to invoke geometric tools, followed by Reinforcement Fine-Tuning (RFT) with reward functions that prioritize computational accuracy and successful task execution.

Our contributions are threefold:
(1) We identify and formalize the distinction between spatial and geometric reasoning in embodied AI, demonstrating that precise robotic manipulation requires computational rather than perceptual capabilities.
(2) We propose \tiger{}, a framework that augments VLMs with Tool-Integrated Reasoning, enabling them to perform exact geometric computations through code generation and execution rather than approximation.
(3) We present \tigerd{} and a two-stage training pipeline (consisting of Supervised Fine-Tuning (SFT) followed by Reinforcement Fine-Tuning (RFT)) that teaches VLMs to recognize geometric reasoning requirements and execute appropriate computational solutions, achieving state-of-the-art performance on geometric benchmarks and enabling millimeter-precision manipulation in real-world robotic systems.


% Recent advancements in Vision-Language Models (VLMs) have revolutionized robotic perception and decision-making, enabling robots to interpret visual scenes and execute tasks based on natural language instructions. However, current VLMs primarily excel in coarse-grained estimations—such as approximate distances, object scales, and basic target identification—which suffice for simple tasks but falter in scenarios demanding precise spatial understanding.

% On the perception side, estimating accurate depth and camera intrinsics from a single image is theoretically impossible without additional priors, leading to insufficient generalization in VLMs due to data limitations. While specialized models for depth estimation exist~\cite{wang2025moge, depthanything, depthanything2, wang2025vggt, wang2025continuous}, their integration into VLMs~\cite{fan2025vlm, wu2025spatial, zheng2025learning} remains suboptimal. In real-world settings, depth sensors or stereo cameras can provide precise depth maps, yet feeding dense pixel-wise depth information into VLMs remains challenging. Existing approaches~\cite{cheng2024spatialrgpt, liu2025ssr, zhou2025roborefer, cai2025spatialbot} that attempt to encode depth information into VLM inputs typically resort to naive solutions, such as normalizing depth values to the 0-255 range and processing them through standard image encoders, which fails to preserve the geometric and metric properties inherent in depth data. Furthermore, in multi-view scenarios, camera extrinsics are often unavailable as inputs, impeding unified scene understanding.

% Regarding output modalities, while a minority of VLMs can output 3D positions or 3D bounding boxes~\cite{team2025gemini}, these predictions are typically data-driven rather than grounded in real-world metric scale; the vast majority of VLMs still produce only 2D pixel coordinates, lacking the capacity to infer metric 3D points, object poses, or rotation angles. This limitation significantly hampers robots’ ability to perform complex manipulation or navigation tasks that demand precise geometric outputs.

% To overcome these barriers, we propose \tiger{}: Tool-Integrated Geometric Reasoning, a novel approach that ``plugs in'' high-precision geometric information into the VLM inference pipeline through Tool-Integrated Reasoning (TIR). \tiger{} empowers robots to self-invoke external tools to retrieve camera intrinsics, extrinsics, and depth data. For computations requiring extensive calculation, the model generates code specifications, invokes code-generation tools, and interprets the returned results to derive target values, thereby bridging the gap between perceptual limitations and actionable robotic outputs.

% We curate a comprehensive dataset, \tigerd{}, consisting of 300K samples synthesized via template-based construction and large-model generation. Starting from a base VLM, we apply Supervised Fine-Tuning (SFT) to align the model with geometric-reasoning tasks, followed by Reinforcement Fine-Tuning (RFT) that incorporates a carefully designed reward function emphasizing accurate tool invocation and metrically correct geometric reasoning.

% Our contributions are threefold:
% (1) We propose \tiger{}, a novel framework that augments VLMs with Tool-Integrated Reasoning to inject precise geometric information into the inference pipeline, transforming spatial estimation into accurate geometric computation.
% (2) We present \tigerd{}, a large-scale dataset of 300K samples with comprehensive tool invocation sequences for training geometric reasoning capabilities in both single and multi-view scenarios.
% (3) We develop a two-stage training pipeline combining SFT and RFT with specialized reward functions for tool-augmented reasoning, achieving state-of-the-art results on multiple spatial benchmarks and enabling high-precision robotic manipulation in real-world environments.
